Rounding Lasserre SDPs using column selection and spectrum-based approximation schemes for graph partitioning and Quadratic IPs

We present an approximation scheme for minimizing certain Quadratic Integer Programming problems with positive semidefinite objective functions and global linear constraints. This framework includes well known graph problems such as Minimum graph bisection, Edge expansion, Sparsest Cut, and Small Set expansion, as well as the Unique Games problem. These problems are notorious for the existence of huge gaps between the known algorithmic results and NP-hardness results. Our algorithm is based on rounding semidefinite programs from the Lasserre hierarchy, and the analysis uses bounds for low-rank approximations of a matrix in Frobenius norm using columns of the matrix. For all the above graph problems, we give an algorithm running in time $n^{O(r/\epsilon^2)}$ with approximation ratio $\frac{1+\epsilon}{\min\{1,\lambda_r\}}$, where $\lambda_r$ is the $r$'th smallest eigenvalue of the normalized graph Laplacian $\mathcal{L}$. In the case of graph bisection and small set expansion, the number of vertices in the cut is within lower-order terms of the stipulated bound. Our results imply $(1+O(\epsilon))$ factor approximation in time $n^{O(r^\ast/\epsilon^2)}$ where is the number of eigenvalues of $\mathcal{L}$ smaller than $1-\epsilon$ (for variants of sparsest cut, $\lambda_{r^\ast} \ge \mathrm{OPT}/\epsilon$ also suffices, and as $\mathrm{OPT}$ is usually $o(1)$ on interesting instances of these problems, this requirement on $r^\ast$ is typically weaker). For Unique Games, we give a factor $(1+\frac{2+\epsilon}{\lambda_r})$ approximation for minimizing the number of unsatisfied constraints in $n^{O(r/\epsilon)}$ time, improving upon an earlier bound for solving Unique Games on expanders. We also give an algorithm for independent sets in graphs that performs well when the Laplacian does not have too many eigenvalues bigger than $1+o(1)$.

==> independent-set.tex <==
Our final algorithmic result is on finding independent sets in a
graph. For simplicity, we focus on unweighted graphs though the
extension for graphs with non-negative vertex weights is
straightforward. We denote by $\alpha(G)$ the size of the largest
independent set in $G$.  Finally we assume $G=(V,E)$ is not a disjoint
union of cycle graphs, i.e. there exists a node $u \in V$ with $d_u\ge
3$ (otherwise the problem is trivial).
%
\begin{theorem}\label{thm:is}
Given 
$0<\eps<1$, positive integer $r$, for any graph $G=(V,E)$ 
with maximum degree $d$,
there exists an algorithm to find an independent set $I\subseteq V$ such that:
\begin{equation}
\label{eq:is-size}
|I|
 \ge  \alpha(G) \cdot \min\left\{
\frac{1}{2 d}
\left(\frac{1}{(1-\eps)\min\{2-\lambda_{n-r-1}(\Lnorm),1\}}
-1\right)^{-1}, 1\right\} 
\end{equation}
in time $n^{O\left(\frac{1}{\eps}\right)} 2^{O(r/\eps^3)}$.
%
%
%
%
%
\end{theorem}
\def\dmax{d}
\begin{remark}
  The above bound \cref{eq:is-size} implies that if $\lambda_{n-r-1}$,
  which is the $(r+1)^{\mathrm{st}}$ largest eigenvalue of the
  normalized graph Laplacian matrix is very close to $1$, then we can
  find large independent sets in $2^{O(r/\eps^2)} n^{O(1/\eps)}$
  time. In particular, if it is at most $1+\frac{1}{4 d}$ where $d$ is
  the maximum degree, then taking $\eps =O(1/d)$, we can find an
  optimal independent set. The best approximation ratio for
  independent set in terms of $\dmax$ is about $O\left(\frac{\dmax
      \cdot \log \log \dmax}{\log \dmax}\right)$
  by~\cite{halldorsson98} and~\cite{halperin02}. The bound
  \cref{eq:is-size} gives a better approximation ratio as soon as
  $\lambda_{n-r-1} \leq 1 + O\left( \frac{1}{\log d}\right)$.  {\hfill
    $\Box$}
%
%
%
\end{remark}
%
\begin{proof}{\it (of \Cref{thm:is})}
 Note that it is not possible to use \Cref{thm:qip} as a black box, 
 while making sure that we find a proper independent set. 
 Instead we will directly use \Cref{cor:faster-qip-main}. 
 %
Consider the following integer program for finding
largest independent set in $G$:
\begin{align*}
\max\qquad & \sum_u \xint_u\\
%
 \st\qquad & 
\xint_u \xint_v = 0 \qquad\mbox{for any edge $e=(u,v)\in E$ ,}\notag
\\
& \xint\in \{0,1\}^{V}.\notag
 \end{align*} 
 Note that we can easily enforce the constraints $\xint_u \xint_v = 0$ 
 by substituting $\xmmt_{\{u,v\}} \gets 0$ in the \lh~relaxation.
%
%
%
%
%
%
%
%
%
%
%

Let $[\xvec_{S(f)}]$ be labeling vectors for moment sequence $\xmmt$ (see~\Cref{prop:mmt-to-labels-k}) and $\xmat=[\xvec_{\{u\}}]_{u\in V}\in \R^{\dims, V}$ be the matrix whose columns are vectors $\xvec_{\{u\}}$ over all $u\in V$. 
Observe that for $A$ and $D$ being adjacency and degree
matrix for $G$ respectively, 
the objective value of above relaxation is: %
\[
\tr(\xmat^T \xmat D^{-1/2} (D+A) D^{-1/2}) = \tr(\xmat^T \xmat).
\]
We will use $\Anorm \triangleq D^{-1/2} A D^{-1/2}$ to denote 
the normalized adjacency matrix so that $\tr(\xmat^T \xmat \Anorm)=0$

At this point, we sample $\xint\sim \bestSfi{}$ as in \Cref{def:best-s-label}. Then we convert $\xint$ into an independent set as follows.
\begin{enumerate}
\item For each $u$, if $\xint_{u}=1$ then let
$I \gets I \cup \{u\}$ with probability $p_u$
which we will specify later. 
\item After the first step, for each edge $e=\{u,v\}$, if $\{u,v\}\subseteq I$, we 
choose one end point randomly, say $u$, and set $I\gets I\setminus \{u\}$.
\end{enumerate}
Finally we output $I$. 
%
It is easy to see that $I$ is an independent set by construction.
%
For any $u$, the probability that it will be included in the final
independent set $I$ is at least:
\begin{eqnarray}
\probs{}{u\in I} & \ge &
\expcts{}{p_u \xint_{u}} -\frac{1}{2}
 \expcts{}{ \sum_{v\in N(u)} p_u p_v \xint_{u}\xint_{v} } \nonumber \\
 & = & p_u \|\xvec_u\|^2 -\frac{1}{2}
 \sum_{v\in N(u)} p_u p_v \langle \Pi_S \xvec_u, \Pi_S \xvec_v\rangle. \label{eq:hwe}
\end{eqnarray}
%
%
By \cref{eq:hwe}, the expected size of the independent set found by the algorithm satisfies
\begin{equation}
\label{eq:ind-set-size}
\expcts{}{|I|} \ge  \sum_u p_u \|\xvec_{u}\|^2 
-\sum_{\{u,v\} \in E} p_u p_v \langle \Pi_S \xvec_{u}, \Pi_S \xvec_{v}\rangle.  
\end{equation} 
Note that for every edge $\{u,v\} \in E$, 
\begin{equation}
\label{eq:vfr-1}
\langle \Pi_S \xvec_{u}, \Pi_S \xvec_{v}\rangle = 
\sum_{f\in \{0,1\}^S} \frac{\langle \xvec_{S(f)}, \xvec_{u}\rangle \langle \xvec_{S(f)}, \xvec_{v}\rangle}{\|\xvec_{S(f)}\|^2} \ge 0 \ . 
\end{equation}
We now consider two cases. 

\medskip
\noindent {\sf Case 1:} $\langle \Pi_S \xvec_{u}, \Pi_S \xvec_{v} \rangle = 0$ for all edges $\{u,v\} \in E$. In this case, we take $p_u=1$ for all $u \in V$, and by \cref{eq:ind-set-size}, we find an independent set of expected size at least $\mu \ge \alpha(G)$. 

\medskip
\noindent {\sf Case 2:} In this case, we have 
\begin{equation}
\label{eq:vfr-2}
 \sum_{\{u,v\} \in E} \langle \Pi_S \xvec_{u}, \Pi_S \xvec_{v}\rangle = \frac{1}{2} \tr(\xmat^T \Pi_S \xmat A) > 0.
 \end{equation}
We define
\begin{equation}
\xi \triangleq \frac{\tr(\xmat^T \Pi_S \xmat \Anorm)}
{\tr(\xmat^T \xmat)}.\label{eq:is-xi-def}
\end{equation}
By \cref{eq:vfr-1,eq:vfr-2}, we have $\xi > 0$.

We now pick $p_u = \frac{\alpha}{\sqrt{d_u}}$ for all $u\in V$, where we will optimize the choice of $\alpha$ shortly.
For this choice, we have
\begin{eqnarray*}
\expcts{}{|I|} & \ge & \alpha \sum_u \frac{1}{\sqrt{d_u}} \|\xvec_{u}\|^2 
-\frac{1}{2} \alpha^2 \tr(\xmat^T \Pi_S \xmat \Anorm)\\
& \ge & \frac{\alpha}{\sqrt{\dmax}} \sum_u \|\xvec_{u}\|^2 
-\frac{1}{2} \alpha^2 \tr(\xmat^T \Pi_S \xmat \Anorm)\\
& = & \mu \bigg(
\frac{\alpha}{\sqrt{\dmax}} 
-\frac{1}{2} \alpha^2 
\underbrace{\frac{\tr(\xmat^T \Pi_S \xmat \Anorm)}
{\tr(\xmat^T \xmat)}}_{\xi}
\bigg)
\end{eqnarray*}
This expression is maximized when $\alpha = \frac{1}{\xi \cdot \sqrt{\dmax}}$, for which it becomes:
\begin{equation}
\expcts{}{|I|} 
\ge 
\frac{\mu}{2 \dmax} \frac{1}{\xi}.\label{eq:eye-size}
\end{equation}
%
%
%
%
We know that for the seed set $\bestS$ chosen by \Cref{cor:faster-qip-main}
satisfies:
\begin{eqnarray*}
\tr(\xmat^T \Pi_S^{\perp} \xmat) + 
\tr(\xmat^T \Pi_S^{} \xmat (I+\Anorm)) & 
\le &  \frac{\tr(\xmat^T \xmat (I+\Anorm))}{\lambda'} \\
&  = & \frac{1}{\lambda'} \tr(\xmat^T \xmat) = \mu 
%
\end{eqnarray*}
where $\lambda' = (1-\eps) \min\{\lambda_{r+1}(I+\Anorm), 1\}
=
(1-\eps) \min\{2-\lambda_{n-r-1}(\Lnorm), 1\}$.

\noindent
On the other hand,
\begin{align*}
%
%
\frac{\tr(\xmat^T \Pi_S^{\perp} \xmat) + 
\tr(\xmat^T \Pi_S^{} \xmat (I+\Anorm))}{\tr(\xmat^T \xmat)} 
= & \frac{\tr(\xmat^T \Pi_S^{\perp} \xmat) + 
\tr(\xmat^T \Pi_S^{} \xmat)+
\tr(\xmat^T \Pi_S^{} \xmat \Anorm)
}{\tr(\xmat^T \xmat)} \\
= & \frac{\tr(\xmat^T \xmat) + 
\tr(\xmat^T \Pi_S^{} \xmat \Anorm)
}{\tr(\xmat^T \xmat)}  = 1 + \xi.
\end{align*}
Thus, for such $\bestS$ we have
$
\xi \le \frac{1}{\lambda'}-1$. Substituting this back into 
\cref{eq:eye-size}:
\[
\expcts{}{|I|} \ge \frac{ \mu }{2 \dmax} \frac{1}{1/\lambda' - 1}.
\tag*{\qedhere} \]

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
\end{proof}

%
%
%
%


==> journal-arxiv.tex <==
\begin{filecontents*}{2csp.tex}
Given a $2$-CSP problem on variables $[n]$ and labels $\labs$, let $G$
be its constraint graph. For convenience, we assume $G$ is regular;
however all our bounds still hold when $G$ is non-regular.  We use $A$
to denote $G$'s normalized adjacency matrix and $\lambda_i$ to denote
the $i^{th}$ smallest eigenvalue of $G$'s normalized Laplacian matrix.
Finally we will use $uv \sim G$ to denote sampling a constraint with
probability proportional to the weight of constraint between $u$ and
$v$.
%
%


\myparagraph{Embedding} 
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
Consider the embedding used in Lemma 5.3 of~\cite{brs11} which is used
to convert $k$ vectors $\xvec_u(i)$ into a single vector.  Given a
partial assignment $f \in \labs^S$ and $u \in [n]$ with $(\xvec_{u\mid
  f}(i))_{i\in \labs} \subset \R^{[m]}$, we define $\xmat_u(f)$ as the
following vector.
%
%
\begin{equation} \label{eq:brs-embed} \xmat_u(f) \triangleq
  \frac{1}{\sqrt{k}} \sum_{j} \frac{(\xvec_{\es\mid f}^{\perp}
    \xvec_{u\mid f}(j))^{\otimes 2}}{\|\xvec_{\es\mid f}^{\perp}
    \xvec_{u\mid f}(j)\|}
  %
  %
  %
\end{equation}
%
%
\myparagraph{Seed Selection and Rounding} 
We will give only an overview of the seed selection procedure.
%
%
%
%
%
%
%
%
%
At $i^{th}$ level, we choose a seed set of size $O(r/\eps)$, $S_i$,
from the matrix $\xmat(f_i) = [\xmat_u(f_i)]_{u\in [n]}$ where
$\xmat_u$'s are defined in~\cref{eq:brs-embed}. After choosing seed
set $S_i$, we sample an assignment $g_i\in \labs^{S_i}$ (conditioned
on $f_{i-1}$) that satisfies
\[
\delta_{f_{i-1},g_i} \le \mathbb{E}_{g \sim \|\xvec_{S\mid
    f_{i-1}}(g)\|^2} \left[ \delta_{f_{i-1},g} \right] \] where
$\delta_f$ is defined in~\cref{eq:brs-delta} and set $f_i \gets
f_{i-1}\circ g_i$. We repeat the seed selection procedure as long as
$\epsilon_{f_i} > \eps$ where $\epsilon_{f}$ is as defined in
\cref{eq:brs-err}.

The rounding procedure remains the same --- independent labeling for
each CSP variable from the respective conditional
distributions. Formally, for each variable $u \in [n]$, we choose a
label $i\in \labs$ with probability $\|\xvec_{u\mid f_i}(i)\|^2$
independently at random.  In~\Cref{thm:brs-final}, we will show that
$\ell = {O}\left( \frac{k^2}{\eps^2} \right)$, i.e. seed selection
will terminate after choosing at most $\ell$ sets.

\myparagraph{Analysis}
Let us begin by defining the quantity
\begin{align}
  \epsilon_{f} \triangleq&
  %
  \mathbb{E}_{uv\sim G} \sum_{(i,j) \in [k]^2}%
  \left| \mathbb{E}\left[ \mathcal{X}_{uv\mid f}(ij) \right] -
    \mathbb{E}\left[ \mathcal{X}_{u\mid f}(i) \right]
    \mathbb{E}\left[ \mathcal{X}_{v\mid f}(j) \right]\right| \notag\\
  = & \mathbb{E}_{uv\sim G} \sum_{i,j}%
  \left| \mathrm{Cov}\left[\mathcal{X}_{u\mid f}(i),
      \mathcal{X}_{v\mid f}(j) \right]\right| %
  %
  %
  = \mathbb{E}_{uv\sim G} \sum_{i,j}%
  \left| \langle \xvec_{\es\mid f}^{\perp} \xvec_{u\mid f}(i),
    \xvec_{\es\mid f}^{\perp} \xvec_{u\mid f}(j) \rangle\right|
  .\label{eq:brs-err}
  %
  %
  %
  %
  %
  %
  %
  %
\end{align}
As shown in \cite{brs11}, the above gives an upper bound on the
expected extra fraction of unsatisfied constraints in the rounded
solution compared to the SDP optimum (when performing rounding after
conditioning on assignment $f$). Therefore, when $\eps_f \le \eps$, we
get an additive $\eps$-error approximation. Our goal is prove (which
we will do in \Cref{thm:brs-final}) that for $\ell \le
\tilde{O}(k/\eps)$, we must have $\eps_{f_\ell} \le
\eps$.  %

\noindent If we define the quantity $\delta_f$ measuring the expected
total variances of each $\mathcal{X}_{u|f}(i)$ as
\begin{equation}\label{eq:brs-delta}
  \delta_f \triangleq 
  \mathbb{E}_u \sum_{i\in [k]} \mathrm{Var}\left[\mathcal{X}_{u\mid f}(i)\right]
  =
  \mathbb{E}_u \sum_{i \in [k]} \|\xvec_{\es\mid f}^{\perp} \xvec_{u\mid f}(i)\|^2 \ ,
\end{equation}
then it is easy to see that $\epsilon_f \le k \delta_f$ by Cauchy-Schwarz. 
%
%

\noindent
We will first relate \cref{eq:brs-err} to the inner products of the
embedded vectors $\xmat_u(f)$.
\begin{claim}%
 \label{clm:brs-lb}
%
 $ \mathbb{E}_{uv\sim G}\left[ \langle \xmat_u(f), \xmat_v(f)\rangle
 \right] \ge \left( \frac{\epsilon_{f}}{k}\right)^2$.
\end{claim}
\begin{proof}
  %
  We have 
  \begin{equation}
    \label{eq:ali09}
    k \langle \xmat_u(f), \xmat_v(f)\rangle 
    %
    = \sum_{ij} \frac{\langle \xvec_{\es\mid f}^{\perp} \xvec_{u\mid f}(i),
      \xvec_{\es\mid f}^{\perp} \xvec_{v\mid f}(j)
      \rangle^2 }{\|\xvec_{\es\mid f}^{\perp} \xvec_{u\mid f}(i)\|
      \|\xvec_{\es\mid f}^{\perp} \xvec_{v\mid f}(j) \|}
    %
    \ge \frac{ \left(
        \sum_{ij} \left|\langle \xvec_{\es\mid f}^{\perp} \xvec_{u\mid f}(i),
          \xvec_{\es\mid f}^{\perp} \xvec_{v\mid f}(j)
          \rangle\right|\right)^2}{\sum_{ij} \|\xvec_{\es\mid f}^{\perp} \xvec_{u\mid f}(i)\|
      \|\xvec_{\es\mid f}^{\perp} \xvec_{v\mid f}(j) \|} 
\end{equation}
where the second step uses Cauchy Schwarz. Since
%
\[ \sum_i \|\xvec_{\es\mid f}^{\perp} \xvec_{u\mid f}(i)\| \le
\sqrt{k} \left(\sum_i \|\xvec_{\es\mid f}^{\perp} \xvec_{u\mid
    f}(i)\|^2\right)^{1/2} \le \sqrt{k} \left(\sum_i \| \xvec_{u\mid
    f}(i)\|^2\right)^{1/2} = \sqrt{k} \] the expected value of the
above lower bound \eqref{eq:ali09} for $uv \sim G$ is at least
$\eps_f^2/k$.
\end{proof}

\noindent We now upper bound the lengths of the embedded vectors.
\begin{claim}
  \label{clm:brs-ub}
  $\|\xmat_u(f)\|^2 \le \sum_{i \in [k]} \left\| \xvec_{\es\mid
      f}^{\perp} \xvec_{u\mid f}(i)\right\|^2$. In particular,
  $\mathbb{E}_u \|\xmat_u(f)\|^2 \le {\delta_f}{}$.
\end{claim}
\begin{proof}
  $ \frac{1}{k} \|\xmat_u(f)\|^2 = \mathbb{E}_{ij} \frac{\langle
    \xvec_{\es\mid f}^{\perp} \xvec_{u\mid f}(i),
  %
    \xvec_{\es\mid f}^{\perp} \xvec_{u\mid f}(j) \rangle^2
  }{\|\xvec_{\es\mid f}^{\perp} \xvec_{u\mid f}(i)\| \|\xvec_{\es\mid
      f}^{\perp} \xvec_{u\mid f}(j) \|} \le \left(\mathbb{E}_{i}
    \left\| \xvec_{\es\mid f}^{\perp} \xvec_{u\mid
        f}(i)\right\|\right)^2 \le \mathbb{E}_{i} \left\|
    \xvec_{\es\mid f}^{\perp} \xvec_{u\mid f}(i)\right\|^2.$
  %
  %
\end{proof}

\noindent Now for fixed $f$ we will upper bound the expected value of
$\delta_{f, g}$ over $g \sim \|\xvec_{S\mid f}(g)\|^2$ in terms of the
projection distance of the embedded vectors from the subspace spanned
by $X_v(f)$ for $v \in S$. (Below, $X_S(f)^{\perp}$ denotes the
projection onto the orthogonal complement of $\mathrm{span} \{ X_v(f)
\mid v\in S \}$.)
%
\begin{claim} \label{lem:brs-pi-to-x} $ \mathbb{E}_{g \sim
    \|\xvec_{S\mid f}(g)\|^2} \left[ \delta_{f,g} \right] \le
  \mathbb{E}_{u\sim G} \left[ \left\| \xmat_S^{\perp}(f)
      \xmat_u(f)\right\|^2 \right]$.
\end{claim}

\begin{proof}
  We know that $ \expcts{g}{ \left\|\xvec_{\es\mid g,f}^{\perp}
      \xvec_{u\mid g, f}(i)\right\|^2 }= \left\| \Pi_{S\mid f}^{\perp}
    \xvec_{u\mid f}(i)\right\|^2$.  Since $\xvec_{\es\mid f}$ is in
  the span of $\Pi_{S\mid f}$
  %
  $\Pi_{S\mid f}^{\perp} \xvec_{u\mid f}(i) = \Pi_{S\mid f}^{\perp}
  \xvec_{\es\mid f}^{\perp} \xvec_{u\mid f}(i)$.  Similarly for any $v
  \in S$ and $j\in [k]$, the vector $\xvec_{\es\mid f}^{\perp}
  \xvec_{v\mid f}(j)$ is in the span of $\Pi_{S\mid f}$.
  %
  %
  %
  %
  %
  By using the same arguments
  from~\Cref{ug-embed-projection-statement}, namely the embedding used
  here preserves linearity, we obtain $ \sum_i \left\|{\Pi}_{S\mid
      f}^{\perp} \xvec_{\es\mid f}^{\perp} \xvec_{u\mid
      f}(i)\right\|^2 \le \left\|\xmat_S^{\perp}(f) \xmat_u(f)
  \right\|^2$.  Taking expectation over $u$ completes the proof.
\end{proof}

\noindent Using the above, we can prove the main claim about the seed
selection procedure, namely that, assuming $\lambda_r$ is close enough
to $1$, the expected variance $\delta_f$ can be reduced by a geometric
factor by conditioning on the assignment to a further $O(r/\eps)$
nodes.
%
\begin{lemma} \label{lem:brs-001} Given $f\in \labs^{S_0}$, positive
  real $\eps>0$ and positive integer $r$ with $\lambda_{r+1} \ge 1 -
  \frac{\eps^2}{2 k^2}$, if $\epsilon_f \ge \eps$ then there exists a
  set of $O(r k^2/\eps^2)$-columns of $\xmat(f)$, $S$ and $g \in
  \labs^S$ such that $\xvec_{S\mid f}(g)\neq 0$ and:
\begin{equation}
  \delta_{f,g}
  \le 
  \delta_f - \Omega\left(\frac{\eps^2}{k^2}\right).
  %
  \label{eq:lem-brs000}
\end{equation}
%
%
%
%
%
\end{lemma}
\begin{proof}
  %
  %
  Let $\rho \triangleq \eps/k$, and $\mu\triangleq \mathbb{E}_u
  \|\xmat_u\|^2$ where for notational convenience we suppress the
  dependence on $f$ and denote $X_u(f)$ by $X_u$.
%
%
%
%
%
%
%
%
%
Observe that \[ \frac{1}{n} \tr\left[ {\xmat}^T {\xmat} A\right] = 
\mathbb{E}_{uv\sim G} \langle \xmat_u, \xmat_v\rangle\ge (\eps_f/k)^2 \ge \rho^2 \]
by~\Cref{clm:brs-lb}. 
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
This implies $\frac{1}{n} \tr\left[ {\xmat}^T {\xmat} L \right] \le
\mathbb{E}_u \|{\xmat_u}\|^2 - \rho^2 = \mu - \rho^2$.
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
From \Cref{lem:markov-bound}, %
we know that volume sampling $O(r/\rho^2)$ columns from ${\xmat}$
yields a set $S$ for which:
\begin{align*}\mathbb{E}_u \|\xmat_S^{\perp}{\xmat_u}\|^2
  \le & \left(1+{O(\rho^2)}\right) \frac{(1/n) \tr\left[ {\xmat}^T
      {\xmat} L \right]}{1-\max(1-\lambda_{r+1},0)} \le
  \left(1+O(\rho^2)\right) \frac{\mu - \rho^2}{1 - \frac{\rho^2}{2}}
  \intertext{Since $\rho\le 1$, we have $(1 - \rho^2/2)^{-1} \le
    \left(1+\frac{3}{4}\rho^2\right)$:} \le &
  \left(1+O(\rho^2)\right)(\mu - \rho^2) \left(1 + \frac{3}{4}
    \rho^2\right)
  \le  \left(1+O(\rho^2)\right)\left(\mu - \frac{\rho^2}{4}\right) \\
  \le &  \mu - \Omega\left(\rho^2\right) \\
  \le & \delta_f - \Omega\left(\rho^2\right) \qquad \mbox{(by
    \Cref{clm:brs-ub})} \ .
  %
  %
  %
  %
  %
  %
  %
  %
  %
  %
  %
  %
  %
  %
  %
  %
  %
  %
\end{align*}
%
%
%
%
By~\Cref{lem:brs-pi-to-x}, $\mathbb{E}_g\left[ \delta_{f,g}\right] \le
\mathbb{E}_u \|\xmat_S^{\perp}\xmat_u\|^2$, which means there exists
$g$ for which $\delta_{f,g} \le \delta_f -
\Omega\left(\frac{\eps^2}{k^2}\right)$.
\end{proof}
%
We put together everything in the following theorem. 
\begin{theorem} \label{thm:brs-final} For $\ell =
  O\left(\frac{k^2}{\eps^2}\right)$, seed selection procedure will
  output a partial assignment $f_{\ell}$ with $\epsilon_{f_{\ell}} \le
  \eps$.
  %
  %
  %
  %
  %
  %
\end{theorem}
%
\begin{remark}[Faster Implementation]
  \label{rem:faster-brs}
  By using the faster solver from~\cite{gs12-fast}, we can implement a
  matching algorithm for~\Cref{thm:brs-final} whose running time is
  $2^{\poly(k/\eps) r} n^{\poly(k/\eps)}$.
\end{remark}
%
\begin{proof}
  Suppose $\epsilon_{f_i} > \eps$ for all $i \le \ell$.  Then
  by~\Cref{lem:brs-001}, for each $i \le \ell$:
  \[
  0\le \delta_{f_{i}} \le \delta_{f_0} - i
  \Omega\left(\frac{\eps^2}{k^2}\right) \le 1 - \Omega\left(\frac{i
      \eps^2}{k^2}\right) \implies \delta_{f_{\ell}} < 0,
  \] which is a contradiction.
\end{proof}
%
%
%
%

